Where Do Vision Language Models Fail at 3D Reasoning?

Vision-language models can get individual judgments right while struggling to recover and consistently use the exact properties of a 3D object. To characterize this gap, we introduce BedBench, a controlled benchmark of thirteen procedurally generated tasks spanning individual judgments and composite answers. Across twelve open-weight and four frontier models, per-color counting exposes a pronounced weakness: humans achieve 93.3% accuracy, compared with 7.2% for the best model. Targeted fine-tuning raises one model's accuracy from 3.0% to 68.6%, but reveals a further difficulty: its answers about the most common colors remain inconsistent with its own per-color counts. Supplying those counts as text improves its judgments, showing that recovering a property does not mean using it consistently. Reasoning, scaling, and added visual cues each improve individual judgments, but none makes exact answers reliable. To locate the difficulty, we probe Qwen3.5-27B: exact per-color counts remain recoverable at the language model's input, yet the model's answers rarely recover them (65.0% for the probe vs. 3.0% for the model). Image-removal controls further show that some apparent successes require no visual evidence. These findings motivate evaluating 3D reasoning by exact correctness, consistent use, and image dependence, rather than accuracy alone. Code and dataset are publicly available: https://github.com/leduckhai/BedBench

==> author.tex <==
Khai Le-Duc*
Nguyen Kim Hai Bui*

An Ngo Xuan, (Texas A&M)
Nam D. Hoang, (independent)

Yueqi Song, (CMU)
Jiarui Liu, (CMU)
Thai Quoc Hoang, (Salesforce)

Fang Wu, (Stanford)
Chris Ngo, 
Terry Jingchen Zhang, (Vector & Oxford)

Mona Diab, (CMU)
Ran Xu, (Salesforce)
Silvio Savarese, (Salesforce & Stanford)
Xiao-Ming Wu

==> figures/arxiv/fig_t5_k_color_all.tex <==
% arXiv version of figures/fig_t5_k_color_all.tex (same content), wrapfig as in arXiv:2608.07645.
\begin{wrapfigure}{r}{0.4\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/fig_t5_k_color_all.pdf}
  \caption{\textbf{All-color subset exact match on \tfivelong{}.} Expected EM over $k$ counts from the full 12-color palette, including zero counts for absent colors, using the same 100 objects at every $k$. Lines average 12 OW models and five runs under Non-Thinking mode; shading gives pointwise 95\% object-bootstrap intervals. Present-color curves appear in Figure~\ref{fig:t5_k_color_present}. \textbf{Takeaway:} Joint outputs outperform factorized outputs across the full palette, alongside their higher absent-color accuracy.}
  \label{fig:t5_k_color_all}
\end{wrapfigure}


==> figures/arxiv/t5_factorized_models.tex <==
\begin{wraptable}{r}{0.4\textwidth}
\centering
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{@{}lrrr@{}}
\toprule
Model & Joint (\%) & Factorized (\%) & $\Delta$ (pp) \\
\midrule
Qwen3.5-0.8B & 44.49 & 70.55 & \textcolor{custom_darkgreen}{$+26.06$} \\
Qwen3.5-2B & 26.63 & 26.61 & \textcolor{red!70!black}{$-0.03$} \\
Qwen3.5-4B & 35.04 & 35.74 & \textcolor{custom_darkgreen}{$+0.70$} \\
Qwen3.5-9B & 15.35 & 34.07 & \textcolor{custom_darkgreen}{$+18.72$} \\
Qwen3.5-27B & 48.22 & 47.49 & \textcolor{red!70!black}{$-0.73$} \\
Qwen3.5-35B-A3B & 30.13 & 36.92 & \textcolor{custom_darkgreen}{$+6.79$} \\
\midrule
Gemma4-E2B & 37.02 & 28.33 & \textcolor{red!70!black}{$-8.69$} \\
Gemma4-E4B & 41.85 & 9.27 & \textcolor{red!70!black}{$-32.58$} \\
Gemma4-26B-A4B & 17.65 & 15.74 & \textcolor{red!70!black}{$-1.91$} \\
Gemma4-31B & 53.55 & 52.53 & \textcolor{red!70!black}{$-1.02$} \\
\midrule
GLM-4.6V-Flash & 28.85 & 27.62 & \textcolor{red!70!black}{$-1.23$} \\
Kimi-VL-A3B & 11.44 & 13.05 & \textcolor{custom_darkgreen}{$+1.62$} \\
\midrule
\textbf{Mean} & \textbf{32.52} & \textbf{33.16} & \textcolor{custom_darkgreen}{$\mathbf{+0.64}$} \\
\bottomrule
\end{tabular}
\caption{\textbf{Joint vs.\ factorized querying on \tfivelong{}.} Present-color exact-count accuracy (\%) under Non-Thinking mode with color inputs, micro-averaged over color--instance pairs with ground-truth count $>0$ across five runs per model. $\Delta$ denotes factorized minus joint accuracy in percentage points. \textbf{Takeaway:} Factorization improves five models and worsens seven, yielding only a \textcolor{custom_darkgreen}{$+0.64$\,pp} average change across the 12 models.}
\label{tab:t5_factorized_models}
\end{wraptable}

==> figures/automaton_reasoning_traces.tex <==
\begin{figure}[H]
\centering
\resizebox{\linewidth}{!}{%
\begin{tikzpicture}[scale=0.2]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [black, thick] (16.6,-29.6) circle (3);
\draw (16.6,-29.6) node {$S$};
\draw [red!70!black, thick] (28.9,-17.6) circle (3);
\draw (28.9,-17.6) node {$\alpha$};
\draw [thick, custom_darkgreen] (28.9,-41.8) circle (3);
\draw (28.9,-41.8) node {$\beta$};
\draw [black, thick] (43.9,-29.6) circle (3);
\draw (43.9,-29.6) node {$\gamma$};
\draw [red!70!black, thick] (56.4,-17.6) circle (3);
\draw (56.4,-17.6) node {$W$};
\draw [red!70!black, thick] (56.4,-17.6) circle (2.4);
\draw [thick, custom_darkgreen] (56.4,-41.8) circle (3);
\draw (56.4,-41.8) node {$C$};
\draw [custom_darkgreen, thick] (56.4,-41.8) circle (2.4);
\draw [black, thick] (8.9,-29.6) -- (13.6,-29.6);
\fill [black] (13.6,-29.6) -- (12.8,-29.1) -- (12.8,-30.1);
\draw [thick, red!70!black] (18.71,-27.5) -- (26.53,-20);
\fill [black] (26.75,-19.69) -- (25.83,-19.9) -- (26.53,-20.61);
\draw [thick, custom_darkgreen] (18.69,-31.63) -- (26.52,-39.4);
\fill [black] (26.77,-39.69) -- (26.55,-38.77) -- (25.85,-39.48);
\draw [thick, dashed, custom_darkgreen] (27.766,-39.024) arc (-160.80214:-199.19786:28.356);
\fill [black] (27.77,-39.02) -- (27.97,-38.1) -- (27.03,-38.43);
\draw [thick, dashed, red!70!black] (30,-20.24) arc (20.51756:-20.51756:26.692);
\fill [black] (30.11,-20.34) -- (29.92,-21.27) -- (30.86,-20.92);
\draw [thick, red!70!black] (26.27,-16.181) arc (269.38986:-18.61014:2.25);
\fill [black] (28.43,-14.65) -- (28.93,-13.85) -- (27.93,-13.84);
\draw [thick, custom_darkgreen] (28.116,-44.684) arc (12.52022:-275.47978:2.25);
\fill [black] (26.13,-42.93) -- (25.24,-42.62) -- (25.46,-43.59);
\draw [decorate=false, red!70!black, thick] (31.24,-19.47) -- (41.56,-27.73);
\fill [black] (41.56,-27.73) -- (41.25,-26.84) -- (40.62,-27.62);
\draw [decorate=false, thick, custom_darkgreen] (31.23,-39.91) -- (41.57,-31.49);
\fill [black] (41.57,-31.49) -- (40.64,-31.61) -- (41.27,-32.39);
\draw [decorate=false, red!70!black, thick] (31.9,-17.6) -- (53.4,-17.6);
\fill [black] (53.4,-17.6) -- (52.6,-17.1) -- (52.6,-18.1);
\draw [decorate=false, thick, custom_darkgreen] (31.9,-41.8) -- (53.4,-41.8);
\fill [black] (53.4,-41.8) -- (52.6,-41.3) -- (52.6,-42.3);
\draw [decorate=false, thick, custom_darkgreen] (46.05,-31.7) -- (54.25,-39.7);
\fill [black] (54.25,-39.7) -- (54.03,-38.79) -- (53.33,-39.5);
\draw [thick, custom_darkgreen] (30.147,-14.875) arc (151.03448:-53.73003:19.637);
\fill [black] (58.94,-40.22) -- (59.89,-40.15) -- (59.29,-39.34);
\draw [thick, red!70!black] (58.923,-19.217) arc (52.9465:-150.25095:19.541);
\fill [black] (58.92,-19.22) -- (59.26,-20.1) -- (59.86,-19.3);
\draw [decorate=false, red!70!black, thick] (46.06,-27.52) -- (54.24,-19.68);
\fill [black] (54.24,-19.68) -- (53.31,-19.87) -- (54,-20.59);
\end{tikzpicture}%
}

\vspace{0.2em}

\begin{tikzpicture}
\node[
    draw,
    align=left,
    rounded corners,
    inner sep=5pt,
    text width=\dimexpr\linewidth-12pt\relax,
    font=\footnotesize
] {
$S$: VLM decomposes the task.\\
$\alpha$: \textcolor{red!70!black}{Bad behaviors:} Color Confusion, Harnessing, Misc, Prior Bias, Reiterating, Wrong Perception.\\
$\beta$: \textcolor{custom_darkgreen}{Good behaviors:} Good Intuition, Good Perception, Good Tactic, Tool Use.\\
$\gamma$: Budget Hit; $W$: Wrong answer; $C$: Correct answer.\\
Color switching at final state: Correct by Luck (\textcolor{red!70!black}{red} $\rightarrow$ \textcolor{custom_darkgreen}{Green}); Think-Answer Mismatch (\textcolor{custom_darkgreen}{Green} $\rightarrow$ \textcolor{red!70!black}{red}).
};
\end{tikzpicture}
\caption{\textbf{State-machine summary of the annotated reasoning traces.} Span-level taxonomy in Table~\ref{tab:annot_taxonomy}. Each trace starts by decomposing the task ($S$), then moves through spans of \textcolor{red!70!black}{bad} ($\alpha$) or \textcolor{custom_darkgreen}{good} ($\beta$) behaviors (self-loops mark consecutive spans of the same class, dashed edges a switch between classes) and ends in a wrong ($W$) or correct ($C$) answer, either directly or after a budget truncation ($\gamma$). \textbf{Takeaway:} A common failure path is \textcolor{red!70!black}{$S \rightarrow \alpha \rightarrow \gamma \rightarrow W$}, and \emph{Wrong Perception} appears in 42 of the 44 incorrect traces.}
\label{fig:thinking_trace_fsm}
\end{figure}

==> images/app_qual/README.tex <==
Self Note:

The figures for dataset examples for D.11 and D.13 have tricky naming, all other tasks name as "tXX\_YYYY\_ex\_ZZ.png" where ZZ is the actual object id.

However, T11 and T13 have 300 samples for 100 objects so current naming use the the sample id for T11 and T13, not object id

This cause no wrong information to the paper, just note here to not panic in the future. Fix the naming when having time.

==> tables/axes_effect.tex <==
\begin{table}[htb]
\scriptsize
\centering
\setlength{\tabcolsep}{8.5pt}
\begin{tabular}{lccc}
\toprule
Task & Baseline & Axes add-on & $\Delta_\text{axes}$ \\
\midrule
\tonelong{} & 29.1 & 27.7 & $\textcolor{red!70!black}{-1.4}$ \\
\ttwolong{} & 58.8 & 54.7 & $\bf\textcolor{red!70!black}{-4.1}$ \\
\tfourlong{} & 27.1 & 26.4 & $\textcolor{red!70!black}{-0.7}$ \\
\tfivelong{} & 0.7 & 0.5 & $\textcolor{red!70!black}{-0.2}$ \\
\tsixlong{} & 70.2 & 69.7 & $\textcolor{red!70!black}{-0.5}$ \\
\tsevenlong{} & 14.0 & 13.7 & $\textcolor{red!70!black}{-0.3}$ \\
\teightlong{} & 58.2 & 57.0 & $\textcolor{red!70!black}{-1.2}$ \\
\tninelong{} & 55.8 & 53.9 & $\textcolor{red!70!black}{-1.9}$ \\
\ttenlong{} & 53.0 & 52.7 & $\textcolor{red!70!black}{-0.3}$ \\
\televenlong{} & 40.9 & 41.8 & $\textcolor{custom_darkgreen}{+0.9}$ \\
\ttwelvelong{} & 52.6 & 52.1 & $\textcolor{red!70!black}{-0.5}$ \\
\bottomrule
\end{tabular}
\caption{\textbf{Effect of coordinate-axis add-ons on accuracy (pp).} Baseline and axes add-on accuracy for the tasks that receive an axes add-on. \textbf{Takeaway:} Axes lower accuracy on 10 of 11 tasks, most on \ttwo{}; only \televen{} gains.}
\label{tab:axes_effect}
\end{table}

==> tables/color_effect.tex <==
\begin{table}[htb]
\scriptsize
\centering
\setlength{\tabcolsep}{8.5pt}
\begin{tabular}{lccc}
\toprule
Task & Baseline & Color add-on & $\Delta_\text{color}$ \\
\midrule
\tonelong{} & 29.2 & 31.8 & $\textcolor{custom_darkgreen}{+2.6}$ \\
\tthreelong{} & 0.2 & 3.7 & $\textcolor{custom_darkgreen}{+3.5}$ \\
\televenlong{} & 40.9 & 43.7 & $\textcolor{custom_darkgreen}{+2.8}$ \\
\ttwelvelong{} & 52.6 & 59.4 & $\textbf{\textcolor{custom_darkgreen}{+6.8}}$ \\
\tthirteenlong{} & 36.2 & 36.8 & $\textcolor{custom_darkgreen}{+0.6}$ \\
\bottomrule
\end{tabular}
% \caption{\textbf{Impact of color add-ons on task accuracy (pp)}. All the tasks receive color add-on are amplifying by color cues with \hyperref[sec:app_dataset_t12]{T12} is the most beneficial task. Instance-level color-present/color-absent panels for \hyperref[sec:app_dataset_t1]{T1}, \hyperref[sec:app_dataset_t3]{T3}, \hyperref[sec:app_dataset_t11]{T11}, \hyperref[sec:app_dataset_t12]{T12}, and \hyperref[sec:app_dataset_t13]{T13} are given in Tables~\ref{tab:qual_color_cue_t1}--\ref{tab:qual_color_cue_t13} (Appendix~\ref{sec:app_qual_visual_cues}).}
\caption{\textbf{Effect of color add-ons on accuracy (pp).} Baseline and color add-on accuracy for the tasks that receive a color add-on. \textbf{Takeaway:} Color raises accuracy on all five tasks, most on \ttwelve{}.}
\label{tab:color_effect}
\end{table}

==> tables/task_overview.tex <==
\begin{table*}[h]
\centering
\scriptsize
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.12}
\begin{tabular}{>{\raggedright\arraybackslash}p{2.35cm} >{\raggedright\arraybackslash}p{2.5cm} >{\raggedright\arraybackslash}p{10cm}}
\toprule
\textbf{Task Group} & \textbf{Task} & \textbf{Description} \\
\midrule
\multirow{5}{*}{\makecell[l]{Aggregate quantity\\and support}}
& \mbox{\tonelong{}} & Count the number of voxels in a single 3D object from 2 perspective views. \\
& \mbox{\ttwolong{}} & Decide whether a candidate container can fully contain the target 3D object. \\
& \mbox{\tfourlong{}} & Count how many distinct colors appear in the object. \\
& \mbox{\tsevenlong{}} & Identify which color occupies the largest number of voxels in the object. \\
& \mbox{\tninelong{}} & Count how many horizontal voxel layers are visible in the rendered object. \\
\midrule
\multirow{3}{*}{\makecell[l]{Compositional\\decomposition}}
& \mbox{\tthreelong{}} & For 2 objects, report shared voxels and voxels unique to each object. \\
& \mbox{\tfivelong{}} & Recover the per-color voxel counts, requiring color-to-part binding rather than a single global count. \\
& \mbox{\tsixlong{}} & Decide whether the object contains a vertical column taller than a threshold. \\
\midrule
\multirow{2}{*}{\makecell[l]{Relational\\structure}}
& \mbox{\teightlong{}} & Decide whether the object's silhouette is horizontally/vertically symmetric. \\
& \mbox{\ttenlong{}} & Decide whether any face-adjacent pair of blocks shares the same color. \\
\midrule
\multirow{2}{*}{\makecell[l]{Cross-view\\geometry}}
& \mbox{\televenlong{}} & Pick the valid or invalid orthographic projection among 3 candidates. \\
& \mbox{\ttwelvelong{}} & Pick which of 2 candidate views matches the object defined by 3 silhouettes. \\
\midrule
\makecell[l]{Multi-object scene\\reasoning}
& \mbox{\tthirteenlong{}} & Pick the valid or invalid silhouette for a multi-object 3D scene.\\
\bottomrule
\end{tabular}
\caption{The 13 BED tasks, grouped by their primary spatial demands. Appendix~\ref{sec:app_dataset_examples} provides rendered examples of every task.
}
\label{tab:task_overview}
\end{table*}


==> tables/visual_addons.tex <==
\begin{table}[H]
    \centering
    \scriptsize
    % \setlength{\tabcolsep}{15pt}
    \begin{tabular}{llcc}
        \toprule
         Task & Default & Color add-on? & Axes add-on? \\
         \midrule\midrule
         \tthreelong{} & $U$ + $A$ & \tickok & \tickno \\
         \midrule
         \tfourlong{} & $C$ + $N$ & \tickno & \tickok \\
         \tfivelong{} & $C$ + $N$ & \tickno & \tickok \\
         \tsevenlong{} & $C$ + $N$ & \tickno & \tickok \\
         \ttenlong{} & $C$ + $N$ & \tickno & \tickok \\
         \midrule
         \tonelong{} & $U$ + $N$ & \tickok & \tickok \\
         \televenlong{} & $U$ + $N$ & \tickok & \tickok \\
         \ttwelvelong{} & $U$ + $N$ & \tickok & \tickok \\
         \midrule
         \ttwolong{} & $U$ + $N$ & \tickno & \tickok \\
         \tsixlong{} & $U$ + $N$ & \tickno & \tickok \\
         \teightlong{} & $U$ + $N$ & \tickno & \tickok \\
         \tninelong{} & $U$ + $N$ & \tickno & \tickok \\
         \midrule
         \tthirteenlong{} & $U$ + $N$ & \tickok & \tickno \\
         \bottomrule
    \end{tabular}
    \caption{\textbf{Visual add-ons partition of tasks.} $C,U,A,N$ denotes colored, uncolored, coordinate axes overlay, and no coordinate axes overlay, respectively. \textbf{Takeaway:} Add-ons are distributed based on each task's default setting and the potential effect of add-on on the task.}
    \label{tab:visual_addons}
\end{table}

==> tables/visual_cue_bootstrap.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{1pt}
\begin{tabular}{lcc}
\toprule
Task & Color & Axes \\
\midrule
\tonelong{} & $[-0.28, +5.65]$ & $[-3.98, +1.13]$ \\
\ttwolong{} & -- & \textcolor{red!70!black}{$[-5.85, -2.42]$} \\
\tthreelong{} & \textcolor{custom_darkgreen}{$[+1.75, +5.58]$} & -- \\
\tfourlong{} & -- & $[-2.60, +1.30]$ \\
\tfivelong{} & -- & $[-0.72, +0.20]$ \\
\tsixlong{} & -- & $[-2.02, +1.08]$ \\
\tsevenlong{} & -- & $[-1.67, +0.98]$ \\
\teightlong{} & -- & $[-3.00, +0.62]$ \\
\tninelong{} & -- & $[-4.00, +0.27]$ \\
\ttenlong{} & -- & $[-1.97, +1.30]$ \\
\televenlong{} & \textcolor{custom_darkgreen}{$[+1.36, +4.25]$} & \textcolor{custom_darkgreen}{$[+0.04, +1.77]$} \\
\ttwelvelong{} & \textcolor{custom_darkgreen}{$[+3.03, +10.6]$} & $[-2.88, +1.87]$ \\
\tthirteenlong{} & $[-0.31, +1.52]$ & -- \\
\bottomrule
\end{tabular}
\caption{\textbf{Bootstrap confidence intervals for visual-cue effects.} Paired bootstrap 95\% intervals for the accuracy difference (pp) from adding color or coordinate axes. Intervals are pointwise, without multiplicity correction; a dash marks tasks without that comparison. \textbf{Takeaway:} Only color on \tthree{}, \televen{}, and \ttwelve{} and axes on \ttwo{} (negative) and \televen{} (positive) have intervals that exclude zero.}
\label{tab:visual_cue_bootstrap}
\end{table}


==> worldflag_HK.tex <==
\begin{flagdescription}{2/3}
% [inner sep=0pt] removes the invisible TikZ padding so it fits perfectly
\node[inner sep=0pt] at (0.5\flaglength, 0.5) {\includegraphics[width=\flaglength]{figures/Flag_of_Hong_Kong.pdf}};

\framecode{}
\end{flagdescription}
